Improving Denoising Diffusion Probabilistic Models via Exploiting Shared Representations

In this work, we address the challenge of multi-task image generation with limited data for denoising diffusion probabilistic models (DDPM), a class of generative models that produce high-quality images by reversing a noisy diffusion process. We propose a novel method, SR-DDPM, that leverages representation-based techniques from few-shot learning to effectively learn from fewer samples across different tasks. Our method consists of a core meta architecture with shared parameters, i.e., task-specific layers with exclusive parameters. By exploiting the similarity between diverse data distributions, our method can scale to multiple tasks without compromising the image quality. We evaluate our method on standard image datasets and show that it outperforms both unconditional and conditional DDPM in terms of FID and SSIM metrics.

==> abstract.tex <==
In this work, we study the multi-task image generation problem using denoising diffusion probabilistic models (DDPM) under limited data regimes. Inspired by representation-based techniques in few-shot learning, we propose a novel DDPM method consisting of shared and exclusive parameters which effectively learns from fewer samples in multi-task schemes. Our algorithm provides a scalable solution by exploiting the similarity between diverse distributions using a core meta architecture (e.g., UNet model) followed by personalized layers. We empirically demonstrate that our proposed method outperforms vanilla DDPM in terms of FID and SSIM metrics on standard image datasets such as MNIST, Fashion-MNIST, CIFAR-10, and CIFAR-100.
